On optimal $L^2$- and surface flux convergence in FEM (extended version)

We show that optimal $L^2$-convergence in the finite element method on quasi-uniform meshes can be achieved if, for some $s_0 > 1/2$, the boundary value problem has the mapping property $H^{-1+s} \rightarrow H^{1+s}$ for $s \in [0,s_0]$. The lack of full elliptic regularity in the dual problem has to be compensated by additional regularity of the exact solution. Furthermore, we analyze for a Dirichlet problem the approximation of the normal derivative on the boundary without convexity assumption on the domain. We show that (up to logarithmic factors) the optimal rate is obtained.

==> numerics_2D.tex <==
\begin{table}[ht]
\begin{center}\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{$(x_0,y_0) = (0,0)$}
&\multicolumn{2}{|c|}{$(x_0,y_0) = (0.5,0)$}
&\multicolumn{2}{|c|}{$(x_0,y_0) = (0,1)$}  \\
\multicolumn{2}{|c|}{$a = 2/3 \pi$}
&\multicolumn{2}{|c|}{$a=\pi$}
&\multicolumn{2}{|c|}{$a=\pi$}  \\
\hline
L2 error  & rate &L2 error  & rate & L2 error & rate  \\ \hline
7.8969e-03 &  -    &1.2069e-02 & -&1.1063e-02&-\\
3.0011e-03  &1.40 &4.1395e-03&1.54&3.5229e-03 &1.65\\
1.1566e-03  &1.38 &1.3543e-03&1.61&1.0832e-03&1.70\\
4.4413e-04  &1.38 &4.3196e-04 &1.65&3.2888e-04&1.72\\
1.7025e-04  &1.38 &1.3569e-04&1.67&9.9264e-05&1.73\\
6.5055e-05  &1.39 &4.2198e-05&1.69&2.9859e-05&1.73\\
2.4769e-05  &1.39 &1.3030e-05 &1.70&8.9609e-06&1.74\\
9.3974e-06  &1.40 &4.0022e-06 &1.70&2.6847e-06&1.74\\
  \hline
\end{tabular}
   \caption{L-shaped domain: Influence of the position of singularity for $\alpha = 0.75$}
%and $a=2/3 \pi$ for $(x_0,y_0) = (0,0)$ and $a= \pi$ for $(x_0,y_0) 
%= (0.5,0)$ and $(x_0,y_0) = (0,1)$}
\label{tab:lshape1}
\end{center}
\end{table}


\begin{table}[ht]
\begin{center}\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{$\alpha = 10/9$}
&\multicolumn{2}{|c|}{$\alpha =4/3$}
&\multicolumn{2}{|c|}{$\alpha = 3/2$}  \\
\hline
L2 error  & rate &L2 error  & rate & L2 error & rate  \\ \hline
1.3295e-02&  -   &1.7801e-02 &  -    & 1.9678e-02 &- \\
4.2329e-03& 1.65 & 5.2865e-03 & 1.75 & 5.5836e-03 &1.82 \\
1.2489e-03&1.76 & 1.4561e-03 & 1.86 &1.4800e-03&1.92 \\
3.5939e-04&1.80 & 3.9056e-04 & 1.90 &3.8327e-04 &1.95 \\
1.0148e-04& 1.82 & 1.0294e-04 & 1.92&9.7928e-05 &1.97 \\
2.8339e-05&1.84 & 2.6855e-05 & 1.94 &2.4843e-05& 1.98 \\
7.8663e-06&1.85 & 6.9612e-06 & 1.95 &6.2773e-06&1.98 \\
2.1779e-06&1.85  & 1.7972e-06 & 1.95 &1.5823e-06 &1.99\\
  \hline
\end{tabular}
   \caption{L-shaped domain: Influence of  $\alpha $ for
     and $a=2/3 \pi$ and $(x_0,y_0) =(0,0)$}
\label{tab:lshape2}
\end{center}
\end{table}



\begin{table}[ht]
\begin{center}\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{$(x_0,y_0) = (0,0)$}
&\multicolumn{2}{|c|}{$(x_0,y_0) = (0.5,0)$}
&\multicolumn{2}{|c|}{$(x_0,y_0) = (0,1)$}  \\
\multicolumn{2}{|c|}{$a = \pi/2$}
&\multicolumn{2}{|c|}{$a=\pi$}
&\multicolumn{2}{|c|}{$a=\pi$}  \\
\hline
L2 error  & rate &L2 error  & rate & L2 error & rate  \\ \hline
5.6427e-03  &  -  &1.5479e-02 & -   &1.1518e-02 & -   \\
2.2076e-03  &1.35 &6.0053e-03 &1.37 &3.8977e-03 &1.56 \\
9.2506e-04  &1.25 &2.1881e-03 &1.46 &1.2592e-03 &1.63 \\
4.0400e-04  &1.20 &7.1529e-04 &1.61 &3.9846e-04 &1.66 \\
1.7782e-04  &1.18 &2.2878e-04 &1.64 &1.2446e-04 &1.68 \\
7.7725e-05  &1.19 &7.2999e-05 &1.65 &3.8538e-05 &1.69 \\
3.3635e-05  &1.21 &2.3250e-05 &1.65 &1.1858e-05 &1.70 \\
1.4428e-05  &1.22 &7.5457e-06 &1.62 &3.6315e-06 &1.71\\
  \hline
\end{tabular}
   \caption{Slit domain: Influence of the position of singularity for $\alpha = 0.75$}
%     and $a=1/2 \pi$ for $(x_0,y_0) = (0,0)$ and $a= \pi$ for $(x_0,y_0) 
%= (0.5,0)$ and $(x_0,y_0) = (0,1)$ }
\label{tab:lshape1}
\end{center}
\end{table}



\begin{table}[ht]
\begin{center}\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{$\alpha = 10/9$}
&\multicolumn{2}{|c|}{$\alpha =4/3$}
&\multicolumn{2}{|c|}{$\alpha = 3/2$}  \\
\hline
L2 error  & rate &L2 error  & rate & L2 error & rate  \\ \hline
1.3303e-02&  -   & 1.6823e-02 &  -   & 1.8589e-02 &  -   \\
3.9682e-03& 1.75 & 4.6200e-03 & 1.86 & 4.8854e-03 & 1.93\\
1.1798e-03& 1.75 & 1.2515e-03 & 1.88 & 1.2627e-03 & 1.95\\
3.4835e-04& 1.76 & 3.3569e-04 & 1.90 & 3.2327e-04 & 1.97\\
1.0291e-04& 1.76 & 8.9685e-05 & 1.90 & 8.2403e-05 & 1.97\\
3.0594e-05& 1.75 & 2.3944e-05 & 1.91 & 2.0960e-05 & 1.98\\
9.1844e-06& 1.74 & 6.3997e-06 & 1.90 & 5.3258e-06 & 1.98\\
2.7892e-06& 1.72 & 1.7142e-06 & 1.90 & 1.3524e-06 & 1.98\\
  \hline
\end{tabular}
   \caption{Slit-shape domain: Influence of  $\alpha $ for
     and $a=1/2 \pi$ $(x_0,y_0) =(0,0)$}
\label{tab:lshape2}
\end{center}
\end{table}


